A Hierarchical Control Framework for Drift Maneuvering of Autonomous Vehicles

Drift control is significant to the safety of autonomous vehicles when there is a sudden loss of traction due to external conditions such as rain or snow. It is a challenging control problem due to the presence of significant sideslip and nearly full saturation of the tires. In this paper, we focus on the control of drift maneuvers following circular paths with either fixed or moving centers, subject to change in the tire-ground interaction, which are common training tasks for drift enthusiasts and can therefore be used as benchmarks of the performance of drift control. In order to achieve the above tasks, we propose a novel hierarchical control architecture which decouples the curvature and center control of the trajectory. In particular, an outer loop stabilizes the center by tuning the target curvature, and an inner loop tracks the curvature using a feedforward/feedback controller enhanced by an $\mathcal{L}_1$ adaptive component. The hierarchical architecture is flexible because the inner loop is task-agnostic and adaptive to changes in tire-road interaction, which allows the outer loop to be designed independent of low-level dynamics, opening up the possibility of incorporating sophisticated planning algorithms. We implement our control strategy on a simulation platform as well as on a 1/10 scale Radio-Control~(RC) car, and both the simulation and experiment results illustrate the effectiveness of our strategy in achieving the above described set of drift maneuvering tasks.

==> curvature-estimation.tex <==
We estimate the curvature of the current trajectory by fitting a curve to the state data from $T$ recent time steps $\left\{x^{(i)},y^{(i)},\dot{x}^{(i)},\dot{y}^{(i)} \right\}_{i=1}^T$. In particular,
we formulate the estimation of curvature $\kappa$, or equivalently, radius $R=\kappa^{-1}$ as the following nonlinear optimization problem:
\begin{align*}
    \arg \min\limits_{x_0,y_0,R} & \sum\limits_{i=1}^{T}\left({R_\text{geo}^{(i)}}^2-{R}^2\right)^2+\left({R_\text{kin}^{(i)}}^2-R^2\right)^2, \\
    \text{s.t. }& R_\text{geo}^{(i)} = \sqrt{\left(x^{(i)}-x_0\right)^2+\left(y^{(i)}-y_0\right)^2}, \\
    & R_\text{kin}^{(i)} = \frac{\sqrt{\left(\dot{x}^{(i)}\right)^2+\left(\dot{y}^{(i)}\right)^2}}{\left|\Dot{\psi}^{(i)}\right|}, \\
    & R = \sum\limits_{i=-T+1}^{0}\frac{R_\text{geo}^{(i)}+R_\text{kin}^{(i)}}{2},
\end{align*}
where $(x_0, y_0)$ is the center coordinate of the estimated circle. An advantage of our algorithm compared to existing circle fitting algorithms~\cite{Kasa1976ACF} is that our algorithm complements geometric information with kinematics information (denoted by $R_\text{geo}$ and $R_\text{kin}$ respectively in the above formulation), which leverages the full power of on-board sensors.


==> feedback.tex <==
We decouple the control of the slip angle $\beta$ and the radius $R$ using two separate PID control loops. In particular, we choose to track a fixed sideslip angle $\beta_{\text{ref}}$, e.g., $\beta_{\text{ref}} = -\pi / 3$ for counter-clockwise drifting, by tuning the steering angle $\delta$, and track a task-dependent target radius $R_{\text{ref}}$ by tuning the wheel rotational speeds. For the rest of this paper, we use the same rotational speed for the front and rear wheels, i.e., $\omega_f = \omega_r = \omega$. As motivated above, we choose different operation frequencies for the two control loops. In our implementation, the frequency of the sideslip angle is set to be $100\mathrm{Hz}$, while that of the radius controller is at $10\mathrm{Hz}$.

==> feedforward.tex <==
In order to speed up the transient processes of the inner control loops, we complement the feedback control with feedforward signals $\omega_{ff}, \delta_{ff}$. We notice that the feedforward signals should depend on i) the parameters in the vehicle dynamics model, especially the tire-ground interaction characteristics; ii) the target value of the controlled variables $R$ and $\beta$.

We observe that the tire-ground interaction characteristics can be almost exclusively described by a friction coefficient. The rationale is that given the current state variables $x,y,\psi,\dot{x}, \dot{y}, \dot{\psi}$ and steering angle $\delta$, the future state trajectory can be predicted once the friction coefficients are known, according to~\eqref{eq:xddot}-\eqref{eq:psiddot}. Furthermore, we observe that in the drifting condition, the relative slipping between the tire and the ground dominates over the velocity of the vehicle, i.e., $\omega_f r_f >> v_{fx}^w, v_{fy}^w, \omega_r r_r >> v_{rx}^b, v_{ry}^b$ in~\eqref{eq:def_sf},~\eqref{eq:def_sr}, which implies that $s_f \approx s_r \approx 1$ in~\eqref{eq:def_s}, and hence according to~\eqref{eq:mf}, we have $\mu_{ij} \approx -s_{ij} / s_i \cdot \mu$, where $\mu = D\sin\left(C\arctan B\right)$ is a chracteristic constant of the tire-ground interaction. Based on the above observations, we can reduce the dependency of the feedforward signal to only two variables, namely the friction coefficient $\mu$ and the target value of the controlled variable, and we can determine this relationship experimentally. Taking the feedforward wheel rotational speed $\omega_{ff}$ as an example, we can set $\omega_{ff}\left(R_{ref}, \mu \right) = \omega_{eq}\left(R_{ref}, \mu \right)$, where $\omega_{eq}$ is wheel rotational speed at the drift equillibrium at the radius $R$ with coefficient $\mu$, which can be approximated by fitting a dataset of various drift equillibria obtained offline. A demonstration of the above described data-driven feedforward design is given in Fig.~\ref{fig:feedforward}, where each blue dot $(R, \mu, \omega_{eq})$ represents an instance of equillibrium, and we can observe that $\omega_{eq}$ approximately exhibits a linear dependence on $R$ and $\mu$. Therefore, we can represent $\omega_{ff}$ as a linear function of $R$ and $\mu$ obtained by performing linear regression using the above data points, visualized as the orange plane in Fig.~\ref{fig:feedforward}.

\begin{figure}[!htbp]
    \centering
    \resizebox{\columnwidth}{!}{
        \input{figures/feedforward.tikz}
    }
    % \includegraphics[width=0.8\columnwidth]{figures/bike_model.tikz}
    \caption{Demonstration of our data-driven feedforward design}
    \label{fig:feedforward}
\end{figure}

Finally, we can identify the friction coefficient $\mu$ online using recent trajectory data, based on least-squares fitting. In particular, we periodically solve the follwing optimization problem to find $\mu$ that best explains the observed data:
\begin{align*}
    \underset{\mu}{\operatorname{min}}\; \sum_{i=-T}^{-1} \ell\left(f\left(\mathbf{X}^{(i)}, \mathbf{U}^{(i)}; {\mu}\right), \mathbf{X}^{(i+1)}\right),
    % \label{eq:loss}
\end{align*}
where $T$ is the window size used for fitting, $\ell$ denotes the $\ell_2$ loss, $f$ denotes the discretized dynamics equations~\eqref{eq:xddot}-\eqref{eq:mf} with $D \sin \left(C \arctan \left(B s_{i}\right)\right)$ replace by $\mu$,
and $\mathbf{X}^{(i)}, \mathbf{U}^{(i)}$ denote the state and input vectors (defined in~\eqref{eq:xu}) at step $i$, where w.l.o.g. we set the index of the current time step to be zero.

==> state-estimation.tex <==
In our system setup, we have access to the following observations: i) the position and attitude $x,y,\psi$ of the vehicle, provided by an off-board global position system; ii) the angular velocity $\dot{\psi}$ of the vehicle, provided by an on-board Inertial Measurement Unit~(IMU). Based on the above measurements, we adopt a Kalman Filter~(KF) to estimate the full state $x,y,\psi,\dot{x}, \dot{y}, \dot{\psi}$. To avoid the influence of inaccurate modeling of the vehicle dynamics, we only use the essential relationship of position, velocity, and acceleration as the model for the KF. Furthermore, to mitigate the influence of the position and attitude measurements being transmitted through a wireless channel subject to random delays and packet drops, we use an asynchronous KF implementation~\cite{async_kf}, which performs update upon the arrival of each new observation from any sensor.

